Experience Recommendation for Long Term Safe Learning-based Model Predictive Control in Changing Operating Conditions

Learning has propelled the cutting edge of performance in robotic control to new heights, allowing robots to operate with high performance in conditions that were previously unimaginable. The majority of the work, however, assumes that the unknown parts are static or slowly changing. This limits them to static or slowly changing environments. However, in the real world, a robot may experience various unknown conditions. This paper presents a method to extend an existing single mode GP-based safe learning controller to learn an increasing number of non-linear models for the robot dynamics. We show that this approach enables a robot to re-use past experience from a large number of previously visited operating conditions, and to safely adapt when a new and distinct operating condition is encountered. This allows the robot to achieve safety and high performance in an large number of operating conditions that do not have to be specified ahead of time. Our approach runs independently from the controller, imposing no additional computation time on the control loop regardless of the number of previous operating conditions considered. We demonstrate the effectiveness of our approach in experiment on a 900\,kg ground robot with both physical and artificial changes to its dynamics. All of our experiments are conducted using vision for localization.

==> src/methodology_f_score.tex <==
\section{METHODOLOGY}

In this section, we present our approach for long-term, safe learning using a combination of experience recommendation and GPs. The purpose of this algorithm is to choose the most relevant experiences to construct a predictive model for the upcoming section of the path that guarantees the assumptions made by the safe controller are valid. We treat each run as potentially belonging to a different mode. 

The approach is based on three steps. First, we construct a GP to model the dynamics for the current run. Then we determine if there are runs that are so different form the current run that adding data from these runs could lead to unsafe model errors. These runs are discarded. From the remaining runs, we check which runs are most similar to the live run and then construct a GP for the dynamics over the upcoming section of the path from the most similar run.

%\begin{itemize}
%	\item Intro paragraph: in this work, we present our approach for AA using X, Y, and Z.
%	\item Subsection for data management
%	\item Subsection for measure of run similarity measure
%	\item Subsection for run rejection (binomial test)
%	\item Algorithm section? putting it all together
%\end{itemize}

\subsection{Gaussian Process (GP) Disturbance Model}
We model the unknown dynamics, $\mb{g}(\cdot)$, as a GP based on past observations. We drop the $(\cdot)^c$ for notational convenience, as we learn a GP for each mode separately. Since there are many good references on GPs \cite{GPforML2006}, here we provide only a high-level sketch. The learned model depends on previously gathered experiences which are assembled from measurements of the state denoted by $\hat{\x}$ and the $\mb{u}$ using \eqref{eqn:MotionModel}, so that 
\begin{align}
    \hat{\mb{g}}(\mb{a}_{k-1}) = \hat{\x}_k - \mb{f}(\hat{\x}_{k-1}, \mb{u}_{k-1}).
    \label{eqn:GeneralExperienceFormula}
\end{align}
The resulting pair, $\left\lbrace\mb{a}_{k-1},\hat{\mb{g}}(\mb{a}_{k-1})\right\rbrace$, forms an individual experience. For simplicity, we model each dimension of the disturbance using a separate GP. Below we derive the equations for a single dimension of $\mb{g}(\cdot)$ denoted by $g(\cdot)$.

A GP is a distribution over functions given past experiences, $\mathcal{D} =\{\hat{g}(\mb{a}_i), \mb{a}_i\}_{i=1}^m$, and kernel hyper-parameters. 

We assume the experiences are noisy observations of the true function $g(\mb{a}_k)$; this is, $\hat{g}(\mb{a}_k) = g(\mb{a}_k) + \eta_{\eta}$ where $\eta_{\eta} \sim \mathcal{N}(0, \sigma_{\eta}^2)$.  The posterior distribution is characterized by a mean and variance which can be queried at any point $\mb{a}_*$ using
\begin{align}
  \label{eqn:GPmean}
  \mu(\mb{a}_*) &=  \mb{k}(\mb{a}_*)\mb{K}^{-1}\hat{\mb{g}},\\
  \sigma^2(\mb{a}_*) &= \kappa(\mb{a}_*, \mb{a}_*) - \mb{k}(\mb{a}_*)\mb{K}^{-1}\mb{k}(\mb{a}_*)^T,
  \label{eqn:GPvariance}
\end{align}
where $\hat{\mb{g}} = [\hat{g}(\mb{a}_1),...,\hat{g}(\mb{a}_m)]^T$ is the vector of observed function values, the covariance matrix $\mb{K}\in\mathbb{R}^{m\times m}$ has entries $[\mb{K}(\mb{a}_i,\mb{a}_j)] = \kappa(\mb{a}_i,\mb{a}_j) + \sigma_{\eta}^2 \delta_{ij}$, where~$\delta_{ij}$ is the Kronecker delta, and the vector $\mb{k}(\mb{a}_*)=[\kappa(\mb{a}_*, \mb{a}_1), ..., \kappa(\mb{a}_*, \mb{a}_m)]$ contains the covariances between the new test point $\mb{a}_*$ and the observed data points $\mathcal{D}$. For this work, we use the squared exponential kernel,
\begin{align}
    \kappa(\mb{a}_i, \mb{a}_j) =\sigma_f^2 \exp\left( - \frac{1}{2 }(\mb{a}_i - \mb{a}_j)^T \mb{L}^{-2}(\mb{a}_i - \mb{a}_j)\right)
    \label{eqn:Kernel}
\end{align}
because of its success in modelling robot dynamics \cite{Ostafew2014ICRA, Ostafew2015ICRA,Ostafew2015RCLBMPC, Berkenkamp2015SafeRobust, Tomlin2012QuadExperiment}. The hyper-parameters are the diagonal matrix, $\mb{L}$, of length-scales which are inversely related to the importance of each element of $\mb{a}$, and the process noise variance, $\sigma_f^2$, which is the variance of the prior family of functions represented by $g(\cdot)$.

As training data is added to a particular GP, uncertainty is reduced and the posterior distribution of the GP specializes to a particular family of functions which represents the system dynamics in a particular mode. The job of the experience recommendation, which is the contribution of this work, is to choose training data that is most relevant to the robots current dynamics.

\subsection{Data Management}

%\begin{figure}
%\centering
%\def\svgwidth{0.475\textwidth}
%\graphicspath{{figs/}}
%\input{figs/ExpRecConceptualDrawing.pdf_tex}
%\caption{Overview of data management for the experience recommendation algorithm. Runs 1-3 are represent previous autonomous traverses of the path and the live run represents the current traverse.  Data is stored at each vertex (triangle) along the path. The solid black triangle represents the position of the vehicle in the live run. The dotted triangle represents the predicted position of the vehicle at the end of the MPC prediction horizon. The vertices outlined in green represent vertices along the recently traversed section of the path in the live run. The vertices outlined in red represent vertices in previous runs along the same section of the path. The vertex outlined in blue represents a vertex ahead of the vehicle from the recommended run.}
%\label{fig:ExpRecConceptualDrawing}
%\end{figure}

\begin{figure}
  \centering
  \includegraphics[width=0.45\textwidth]{figs/robochunk_data_with_live_run.pdf}
  \caption{Runs 1 and 2 represent previous autonomous traverses of the path and the live run represents the current traverse. The solid circle indicates the current position of the vehicle and the dotted circle indicates the predicted position of the vehicle at the end of the MPC prediction horizon. Data, $\mathcal{D}_r^v$, for each run, $r$, is stored in small sets at each vertex, $v$, represented by a circle. The goal is to use recent data from the live run (solid box) to construct a GP to assess the similarity to data from previous runs along the corresponding section of the path (dashed box). This is used to recommend experiences from a run with similar dynamics (dotted box) to construct a predictive model for the dynamics on the upcoming section of the path.}
  \label{fig:ExpRecConceptualDrawing}
\end{figure}

The repetitive path following nature of our task greatly restricts the possible motions that the vehicle is likely to take at any point along the path. In addition, the location along the path naturally encodes the path geometry and terrain type. For this reason, we only consider experiences in the region of the path that the vehicle is currently traversing to construct the GP.  To choose the data points for constructing the GP, we divide local data around the vehicle into three subsets (see Fig.  \ref{fig:ExpRecConceptualDrawing}). 

First, let the recent run be run $n$. Recent data from the live run, $\mathcal{D}_n^-$, is used to construct a GP that represents the current dynamics, $\hat{g}_n^-$. We use a sliding window of the last $n_v$ vertices in the path. Experiences older than this are considered no longer relevant to the dynamics on the upcoming section of the path.

Second, data from previous runs over the same section of the path, $\mathcal{D}_i^-, i = 1..n-1$, is used to identify which runs are similar to the current run. Since we assume that the configuration is constant over short periods of time, experiences from runs that are similar to the live run over the previous section of the path are therefore also likely to be relevant to the live run over the upcoming section of the path.

Third, data from the run that is most similar to the current run in window ahead of the vehicle, $\hat{\mathcal{D}}_n^+$, is added to the local GP that will be used for control.

%\begin{enumerate}
%	\item A GP is constructed using recent data from the live run (green) and is used as a generative model for the current dynamics over this section of the path. Let this be the live GP.
%	\item Data is pulled from Robochunk from all previous runs along the recently traversed section of the path (red). This data consists of the measured input/output pairs for each run that correspond to the GP input and associated model error which is the regression target.
%	\item A prediction is made using the live GP for each input in each previous run. This gives a predicted mean and standard deviation for each output in each run.
%	\item These input/output/prediction tuples are used to measure the similarity between the live run and each previous run (see Section \ref{sec:RunSimilarity}). Any run that is too different from the live run is rejected entirely to preserve an accurate bound on model error (see Section \ref{sec:RunRejection}).
%	\item Points are drawn from a vertex ahead of the vehicle from the most similar run (blue) until the desired number of new points has been reached. If not enough points are available from the most similar run, points from the next most likely run are used until the desired number of points has been reached or no more runs are available.
%\end{enumerate}

% Binomial test
\subsection{Run Rejection Criteria}
\label{sec:RunRejection}

The controller uses the $3\sigma$ bounds on the prediction from the GP as an upper bound on the model error. It is therefore important to ensure that these bounds are correct. 

Before considering a previous run, $i$, as a candidate to draw sample from for $\hat{\mathcal{D}}_n^+$, we test whether the proportion of samples from $\mathcal{D}_i^-$ that lie outside of the predicted $3\sigma$ bounds from $\hat{g}_n^-$ is significantly higher than would be expected by chance. We do this using the binomial test.

Let $N$ be the number of input-output pairs in $\mathcal{D}_i^-$ and $n$ be the number of outliers according to the predictions from $\hat{g}_n^-$. We use a Binomial distribution $B(x,N, p)$ to calculate the probability of $n$ or more outliers in a sample of size $N$ if the true probability of drawing an outlier is $p$. This is given by
\begin{equation}
	p(\text{number outliers $> n$}) = \sum_{x=n}^{N}B(x,N,p).
\end{equation}
We reject the run if $p(\text{number outliers $> n$})  < \alpha$. We chose a $5\%$ significance level for our experiments so that there is at least a 95\% chance that the $3\sigma$ bounds will be a good upper bound for the model error.

% Note that this will only be effective where the GP has data in the same input region as the run being tested. Otherwise the variance of the GP for the live run will be close to the GP prior which does not have strong discriminating power. In other words, this test only rules out runs where we have strong evidence to support that the two runs are different.

\subsection{Run Similarity Measure}
\label{sec:RunSimilarity}

This section describes our method for determining which data to include in the GP for modelling the dynamics over the upcoming section of the path. The goal of this step is to identify which runs are most similar to the current run given recent data from the live run and data from previous runs over the same section of the path.

The likelihood ratio test was chosen because of its good performance on test data relative to several alternatives including the KL-divergence, the Anderson-Darling test, and the likelihood of data from each run given $\hat{g}_n^-$. A similar test is used in computational biology to determine two genetic sequences are aligned \cite{Eddy2008SeqAlignment}. The test is based on the assumption that data comes from either the same process as the live run (modelled as a GP using recent data) or from random noise (modelled as the GP prior). The runs with the highest likelihood ratio are most similar to the live run compared to the GP prior.

Let $\hat{g}_0$ be the GP prior. The GP prior and $\hat{g}_n^-$ form the two hypothesis distributions. Next, we compute the forward score, $F_i$, for each run, $i$, using the likelihood of data from that run over the recently traversed portion of the path $\data_i^-$,
\begin{equation}
	F_i = \log \frac{p(\data_i^-|\hat{g}_n^-)}{p(\data_i^-|\hat{g}_0)}
\end{equation}

The posterior probability of model $\hat{g}_n^-$ given data $\data_i^-$ is then given by evaluating a sigmoid function of $F_i$. We found that the posterior can reach one for multiple runs due to numerical precision, so we use $F_i$ instead. As in our previous method \cite{McKinnon2017MMLearning}, runs that are more similar to the prior than the live run ($F_i < 0$) are considered not relevant to the current run and rejected from further consideration.

\rtext{FOR ANGELA: } The issue we talked about comes from the fact that $F_i$ depends on the number of data points in each run which varies between runs. Let $N$ be the number of points in $\data_i^- = \left\lbrace (g_j, a_j); j=1..n\right\rbrace$.
\begin{align*}
	F_i &=  \log \frac{p(\data_i^-|\hat{g}_n^-)}{p(\data_i^-|\hat{g}_0)}\\
	      &= \log \left( \frac{\prod_{j=1}^N p(g_j|\hat{g}_n^-(a_j)}{\prod_{j=1}^N p(g_j|\hat{g}_0(a_j))} \right)\\
	      &=  \log \left( \prod_{j=1}^N \frac{p(g_j|\hat{g}_n^-(a_j)}{p(g_j|\hat{g}_0(a_j))}\right)\\
	      &= \sum_{j=1}^N \log \left( \frac{p(g_j|\hat{g}_n^-(a_j)}{p(g_j|\hat{g}_0(a_j))}\right)\\
	      &=N\bar{F}_i
\end{align*}
where $\bar{F}_i$ is the mean score per point for run $i$. Therefore, the score depends linearly on the number of points in the run. The second line assumes samples are independent. The third and fourth lines are just factoring. This wouldn't be a problem if we fitted a GP to each run (or pseudo-random subset of runs). Then we could get a proper posterior distribution over runs given recent data from the live run. This would be theoretically the most sound, but would be computationally more expensive in its vanilla version.

Our options are:
\begin{enumerate}
	\item Leave the current implementation and just drive at the same speed all the time. This should work for the 1.5 m/s case I showed you on Friday.
	\item Normalize by the number of points to get $\bar{F}_i$.
	\item Fit a GP to each run and do the principled thing. This would be a good comparison anyway and if we had more time, I would definitely do it. It shouldn't be relatively easy to implement too.
\end{enumerate}

\subsection{Overview of the Algorithm}

Putting the components above together, we arrive at the following algorithm.

\begin{algorithm}[H]
\caption{Overview of the experience recommendation algorithm.}
\label{alg:ExperienceRec} 
\begin{algorithmic}
  \State $n \gets$ live run number
  \State $\alpha \gets$ significance level for binomial test
  \State $\mathcal{D}^- \Leftarrow \left\lbrace \mathcal{D}_i^-, i=1..n-1 \right\rbrace$ \Comment{data from candidate runs}
  \State $\hat{g}^-_{n} \gets$ Fit a GP to $\mathcal{D}_n^-$
  \State $scored\_runs = \left\lbrace \right\rbrace$
  \For{$i=1..n-1$} 
  	\State $\mathcal{A}_i^-, \mathcal{G}_i^- \gets$ GP inputs from $\mathcal{D}_i^-$, GP outputs from $\mathcal{D}_i^-$
    \State $\left\lbrace \hat{\mu}_i^-, \hat{\sigma}_i^- \right\rbrace \gets \hat{g}_n^-(\mathcal{A}_i^-)$ \Comment{predicted mean and variance}
  	\State $p_b \gets$ Binomial test probability given $\left\lbrace \hat{\mu}_i^-, \hat{\sigma}_i^-\right\rbrace, \mathcal{G}_i^-$
    \If{$p_b < \alpha$}
    	\State \textbf{continue}
    \EndIf
    \State $F_i \gets$ forward score for run $i$
    \State Append ($i$, $F_i$) to $scored\_runs$
  \EndFor
  \State \textbf{return} $scored\_runs$ sorted from lowest to highest $F_i$.
  % \State $\mathcal{A}_*^+, \mathcal{G}_*^+ \gets$ The desired number of experiences from previous runs starting from the run with the lowest $A^2_i$
  % \State $g^+_{n} \gets$ Fit a GP to the recommended experiences, $\mathcal{A}_*^+, \mathcal{G}_*^+$
\end{algorithmic}
\end{algorithm}

% \subsection{COMPUTATIONAL COST ANALYSIS?}
% SHOULD I SHOW USING $O(\cdot)$ that the proposed method is faster than constructing a GP for each run or will people take this for granted?

% This section illustrates the computational cost savings of the proposed approach compared to our previous approach \cite{McKinnon2017MMLearning}, if we were to use a local GP for each candidate run. Let $n_r$ be the number of candidate runs, $n_{gp}$ be the number of samples in each GP, and assume that the number of samples in each $\mathcal{D}_i^-$ is $n_{gp}$. The computational cost of our previous approach would be $O(n_rn_{gp}^3)$ for fitting $n_r$ GPs and $O(n_rn_{gp}^2n_{gp})$ for evaluating each of the $n_r$ GPs at the $n_{gp}$ most recent data points in the live run. The total cost is then $O(n_r























